Formal Methods for An Iterated Volunteer's Dilemma

Game theory provides a framework for studying communication dynamics and emergent phenomena arising from rational agent interactions. We present a model framework for the Volunteer's Dilemma with four key contributions: (1) formulating it as a stochastic concurrent nn n-player game, (2) developing properties to verify model correctness and reachability, (3) constructing strategy synthesis graphs to identify optimal game trajectories, and (4) analyzing parameter correlations with expected local and global rewards over finite time horizons.

==> 4_timeline.tex <==
\section{Project Timeline}

\input{tables/timeline}

\section{Questions}
\begin{enumerate}
    \item Are stochastic games analogous with nondeterministic games? In its classical form, the Volunteer's Dilemma doesn't appear to have nondeterminism, for example: If $v_0$ chooses to donate their resource, and all other nodes choose to freeride, we move from an initial state of $<0,0,0,0>$ (init state) to $<1,0,0,0>$ with probability of 1, as it doesn't seem to make sense for $v_0$ to take action donate, and instead freeride. Perhaps it would make sense to inject nondeterminism into the model. \cite{6900564} attempts this as a means to dynamically adapt in an iterated version of the Prisoner's Dilemma. Open to feedback here. 
    \item Even if nondeterminism is present, actions are taken concurrently and the environment is only partially observable. We've read about this problem being studied through the lens of Bayesian Inference to model partially observable Markov Decision Processes for other games, but that's likely beyond our scope in the next few weeks.
    \item Does it make sense for each player to act the same, in terms of transition functions? In a real-world setting, there are likely agents with a higher propensity for altruistic behavior, and vice versa.
\end{enumerate}

==> equations/reward_eqs.tex <==
\begin{equation*} \label{eq:1}
r^{k}_i = \begin{cases}
0 & \text{if } \sum_{i=1}^{n} s^{k}_{i'} < r_{needed} \\[6pt]
\frac{r_{needed} \cdot f}{|V|} & \text{if } \sum_{i=1}^{n} s^{k}_{i'} = r_{needed} \\[6pt]
\frac{r_{needed} \cdot f - 0.014(\sum_{i=1}^{n} s^{k}_{i'} - r_{needed})}{|V|} & \text{if } \sum_{i=1}^{n} s^{k}_{i'} > r_{needed}
\end{cases}
\end{equation*}

\begin{equation} \label{eq:2}
R_{i}^{k} = \sum_{i=1}^{n} r^{k}_i
\end{equation}

\begin{equation} \label{eq:3}
c^{k+1}_{i} \leftarrow \min\left(r_{max}, \left\lfloor c^{k}_{i} - s^{k}_{i'} + \frac{R_{i}^{k}}{|V|} \right\rfloor\right)
\end{equation}

==> tables/params.tex <==
\begin{table}[H]
\centering
\caption{Volunteer's Dilemma Parameters}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{2cm}|p{8cm}|}
\hline


Parameter & Definition \\ \hline
$k$ & We refer to rounds of the finite length game as episodes. $k \in \{1,2,3,..., k_{max}\}$ \\ \hline

$k_{max}$ & The maximum number of episodes specified as input into the environment.\\  \hline

$V$ & The set of agents within a system. The game is typically played with $|V| > 2$ in literature\\ \hline

$r$ & The initial allocation of a resource. Each agent within the system is initialized with $r$ = 1 at each episode. A resource could be generalized to be currency, votes or public goods, etc. \\ \hline

$r_{needed}$ & A specified parameter that dictates the number of resources needed to 'win' the game. In the traditional game, only a single volunteer is needed. $r_{needed} \leq |V|$ \\ \hline

$A$ & The action space. $\{a_{donate}, a_{freeride}\} \in A$.  \\ \hline
% Modeling this as a stochastic game would seemingly dictate that each agent has a uniformly distributed strategy vector: $p_{a_{donate}} = p_{a_{freeride}} = 0.5$..

\end{tabular}
}
\end{table}

==> tables/state_space.tex <==
\begin{table}
    \centering
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        Params [kmax, rinit, rneeded] & Players & States & Choices  & Transitions \\ \hline
        [0,100,200] & 3 & 2 & 2 & 2 \\ \hline
        [1,100,200] & 3 & 29 & 55 & 55 \\ \hline
        [2,100,200] & 3 & 732 & 1460 & 1460 \\ \hline
        [3,100,200] & 3 & 16429 & 35435 & 35435 \\ \hline
        [4,100,200] & 3 & 349081 & 776209 & 776209 \\ \hline
    \end{tabular}
\end{table}

==> tables/timeline.tex <==
\begin{table}[H]
\centering
\caption{Project Timeline}
\begin{tabular}{|l|l|}
\hline

Beg. Date & Task \\ \hline
31-Mar & Project Proposal \\ \hline
7-Apr & Formalize Model and adjust to given feedback. \\ \hline
14-Apr & Construct Model in PRISM or Z3 SMT Solver \\ \hline
21-Apr & Write Properties, run simulations \\ \hline
24-Apr & Analyze and synthesize results \\ \hline
27-Apr & Final Project Presentation \\ \hline
1-May & Final Project Report \\ \hline
1-May & Final Project Video Demo\\ \hline

\end{tabular}
\end{table}
